Online Group-exercises for Older Adults of Different Physical Abilities

In this paper we describe the design and validation of a virtual fitness environment aiming at keeping older adults physically and socially active. We target particularly older adults who are socially more isolated, physically less active, and with less chances of training in a gym. The virtual fitness environment, namely Gymcentral, was designed to enable and motivate older adults to follow personalised exercises from home, with a (heterogeneous) group of remote friends and under the remote supervision of a Coach. We take the training activity as an opportunity to create social interactions, by complementing training features with social instruments. Finally, we report on the feasibility and effectiveness of the virtual environment, as well as its effects on the usage and social interactions, from an intervention study in Trento, Italy

==> background.tex <==
% !TEX root = main.tex

\section{Idea Management}

Idea Management (IM) is the process by which organizations approach their communities of clients, employees, suppliers, and interested stakeholders to (1) request ideas, (2) collect and (3) evaluate them, and (4) select the most promising ones to source their innovation needs or to address a defined organization's problem \cite{baumgartner2008introduction}.

The execution of IM processes can be supported by specially-designed software tools known as IM systems. In such systems, organizations can describe an innovation problem they want to solve (e.g., innovate the public transportation system) and setup campaigns through which collect proposed solutions. At the same time, IM systems let users suggest ideas as well as evaluate and place opinions on other users' ideas. 

\subsection{IdeaScale}

We specifically consider the case of IdeaScale\footnote{\url{https://ideascale.com}} as idea management platform. IdeaScale is one of today's leading technologies for supporting the execution of IM processes and used by big companies like Microsoft and Xerox, and by emblematic institutions such as NASA and White House.

In IdeaScale, ideation initiatives are created by setting up a community website in which organizers describe the goals of the initiatives and define campaigns through which ideas are collected. To submit an idea, users, previously registered as member of the community, have to provide a title, description, and associate a campaign to the idea. Optionally, they can label the idea with tags and attach an image or file to enrich the description.

\begin{figure}
\centering
\includegraphics[width=0.55\textwidth]{figures/ideascale_ui-with_ideation-letters}
\caption{(a) Snapshot of a community's website; (b) Idea submission features; (c) Detailed view of an idea, commenting and voting functions}
\label{fig_ideascale}
\end{figure}

Members can also comment and assign positive/negative valuations (votes) to others' ideas and comments. They can also reply to existing comments. These functionalities enable them to not only set their positions regarding the ideas and comments but also to help in refining the content of the proposals. Figure \ref{fig_ideascale} illustrates the described features of IdeaScale.

%By default ideas are listed in three forms in IdeaScale. First, in a chronological order where the newest ideas appear first and the oldest occupy the last positions. Then, by popularity where ideas with highest scores ---scores are calculated by computing the difference between positive and negative votes-- are presented at the top of the list and third by the number of comments gathered by ideas.

==> introduction.tex <==
% !TEX root = main.tex

\section{Introduction}

The increasing competitiveness of the markets forces organizations to sustain a continuous process of innovation fueled with ideas originated from managers, employees and, for some time now, even from outside the organization. Idea Management (IM) is the process of requesting, collecting, selecting and evaluating ideas to develop new, innovative products, services or regulations, or to improve existing ones \cite{baumgartner2008introduction}. The goal of IM is to capture ideas that can deliver benefits to the organization by leading to innovations or by solving specific problems \cite{westerski2011road}.

The emergence of social and collaborative web-based technologies has transformed the physical suggestion boxes ---the former preferred method to listen to customers--- into dedicated IM platforms, which lets people propose ideas, as well as rate and place comments on other users' suggestions \cite{hrastinski2010review}. Examples of popular IM platforms are IdeaScale (\url{http://ideascale.com}), Crowdicity (\url{http://crowdicity.com}), Spigit (\url{http://www.spigit.com}). The offerings and market are growing.

The adoption of IM practices and platforms have been empowering various innovation initiatives around the world. Almost 200,000 people have been participating in My Starbuck Idea, the world-wide IM initiative conducted by Starbucks to collect ideas from its customers about future products and services \cite{schoultz2012starbucks}. Similar participation rates can be found when analyzing Idea Storm, the IM initiative sponsored by the giant computer company Dell \cite{di2009steal}. But, its application has not been limited only to commercial domains. In the political and civic domain, the Icelandic participatory constitution-writing process represents an emblematic case. Here, the population at large has been invited to contribute to the constitution draft with suggestions, proposals, and ideas \cite{landemore2015inclusive}.

About communities
What communities
Who uses  
How it is used 
- collectively
- level of individual users

Why is it important
it is a trend
nothing in the literature -> practice 

Are there clearly defined collective behaviors? 

How the characteristics of the communities are related to collective behavior of the community and users? 

==> relatedworks.tex <==
% !TEX root = main.tex

\section{Related Works}
IM has been playing a key role in efficiently managing grassroots innovation initiatives \cite{bakker2010idea}. In this context, IM platforms have proven able to properly instrument campaigns for soliciting ideas from large-scale crowds, both in the business and the public sector \cite{bailey2010s}. Discussions on how to extend and improve online IM platforms and similar have taken different directions among industrial and academic researchers, from methods to define suggestions, to mechanisms to display streams of ideas, to features to assess proposals, to solutions to find promising contributions \cite{westerski2013semantic}.

Deliberation maps have been presented in \cite{klein2008supporting} to structure participants' contribution as problem trees containing the problem to solve, potential solutions, and arguments for and against proposed solutions. The use of semantic technologies has been proposed by Westerski et al. to organize, link and classify the proposed ideas using meta data annotations \cite{westerski2010model}. Improving scoring methods used to rate the ideas has been the goal of Xu et al. who have proposed a reference-based scoring model as an alternative to the traditional thumbs up/down voting systems \cite{xu2012reference}. Faridani et al. have introduced a two-dimensional visualization plane as an approach to address the filter-bubble effect ---narrowing the exposure to recent, popular, or controversial information--- of linear listings used to display opinions in online sites \cite{faridani2010opinion}. 

Convertino et al. have targeted information overload in the evaluation phase by employing natural language processing methods to automatically identify the core of the proposals \cite{convertino2013idea}. Along this line, Bothos et al. have introduced the application of information aggregation markets to facilitate the evaluation of the ideas \cite{bothos2008collaborative}. From an analytical perspective, \cite{bjork2009good} has employed social network analysis techniques to study the relationship between the quality of the ideas and the connectivity (degree centrality) of the contributors.

Social sharing features, e.g., share and tweet buttons, have been the preferred approach to integrate IM platforms and social networking sites. These solutions have been proposed to quickly and easily export content of IM discussions into general purpose social networks (e.g., Facebook, Twitter) for creating awareness, gaining visibility, and attracting new participants. Although pervasively used across the Internet in general and in IM platforms in particular, their effectiveness to actually increase participation and productivity in IM initiatives have been lately put in doubt \cite{saldivar2016effectiveness}. Alternatively, IdeaScale and Spigit ---two of the big players in the field have proposed solutions that extend Facebook's native features proving IM-specific features, e.g., voting mechanisms, filtering, tagging, and searching functionalities \cite{ideascale2013facebook, spigit2013facebook}. 

Through an application that enhanced Facebook with deliberation functionalities (e.g., survey features, polling tools, moderation capabilities), Bendor et al.  have examined the suitability of Facebook discussion groups to engage the public in conversations about the innovation of Vancouver's public transportation \cite{bendor2012s}. Their promising results provide further support to the idea of using Facebook to carry out product/service innovation initiatives.

==> sections/discussion.tex <==
\section{Discussion}
%Group exercising for older adults of potentially different abilities present many challenges. In this paper we addressed the following aspects. 
%The results presented in the previous sections can be summarised as followed

\subsection{Usability and technology acceptance}
The design proposed in this paper entailed a set of features that added to the complexity of the tool with respect to a more traditional home-based training application. Given the target population, we set to investigate how older adults would react to this added complexity and how their impressions would change over time.
Two different versions of the Trainee application were tested: one supporting a traditional home-based exercise program (Control group) and the other representing the proposed virtual group exercising (Social group). 
%The social group was exposed to a more complex version 

Not surprisingly, the usability of the application was lower for the Social group at the beginning of the study, reflecting participants’ initial difficulties to deal with a more complex user interface. However, over time, usability improved more in the Social group than in the Control group, suggesting that, although the social application was perceived as more complicated at the beginning, perceived usability increased after the training program, approaching the top end of the scale.

The results on technology acceptance were more controversial. The analyses suggested a general improvement of the dimensions related to technology acceptance, especially for the Social group. However, one of the limitations of the study was the small sample size and the subsequent limited statistical power. To overcome this constraint, we used matched random assignment to allocate participants to conditions, combined with a closer exploration of the data analysing both the studentized residuals to examine the error variance of specific cases and the Cook's distance, to measure the overall influence of single cases on the model \cite{field2013discovering}. %Nevertheless, more conclusive results could be obtained with further investigation with larger sample size and higher statistical power.

Overall, while Internet connection was an intermittent issue, both usability and technology acceptance of the Trainee application (both versions) generally improved. 
For the full application, these results mean that 
users could handle the extra complexity and learn to use this type of tool.


\subsection{Design dimensions and user feedback}
A set of design dimensions were derived from previous experiences and literature on home-based training. These dimensions were materialised in Gymcentral and tested in the eight-weeks intervention study. 
The user feedback on the features of each dimension \emph{reinforces the value of group exercising, social interactions and persuasion} features. 

The results also give us more insights on the socialisation aspects. Participants regarded as highly useful the interactions with the Coach, followed by the interactions with the community as a whole, and to a lesser extent the private messages with other trainees. These results, along with the analysis of the individual interactions, point to the need for more effective mechanisms to motivate social interactions among community members. 

From the virtual environments we learned that participants enjoyed seeing each other, and this was particularly true for the Classroom where the participants were engaging of an activity together (i.e., training). Seeing each other and interacting in the Locker room was not perceived as very useful, potential reasons being: lacking activities that would motivate users to stay in the room, contextual messages not being expressive enough, or not being used to real-time messages.

Based on these results, we are currently extending the Virtual Gym to include \emph{environments} that would offer social activities (e.g., listening to music or watching videos) that would motivate users to interact and build stronger relationships 

\subsection{Nature of social interactions}

Qualitative analysis on the social features showed that both participants and the Coach used the bulletin board and private messages differently. %First, private messages were used more extensively than the bulletin board, 
%especially by the Coach to support participants, and to exchange information about technical issues with the application.

Community building activities were of primary importance, especially in the bulletin board where participants played a central role. This suggests that, besides the training, they were also involved in strengthening social interactions with each other, using humour to enhance their relationships, and the bulletin board was the preferred channel. 

When talking about physical activity, participants tended to publicly support and congratulate each other on the bulletin board, while rarely doing so in private. Private conversations were directed mostly to the Coach to discuss personal experiences with the training. Not surprisingly, the Coach was the user who most engaged in these discussions.

Regarding the application, putting aside the messages about problems, the bulletin board was used to express satisfaction whereas private messages for information or questions. 
%Similarly, private messages were used to discuss and exchange information about problems with the application. Participants also tended to use more the private messages for self-disclosure, talking about their lives outside of the virtual gym.

%The coach was very central both in the bulletin board, congratulating publicly with participants for their results with the training, and in private messages, individually motivating them to exercise. The different use he made of the social features suggests different purposes: the public acknowledgement of participants’ achievements in the training to foster motivation in the entire group, and the private support to push individuals to exercise.

These results highlight the need for having both type of channels, since they serve very different purposes. On one hand allowing for community building in public channels, and for more personal conversations in private. We should also note that compared to other technology-based interventions, where social features (e.g., forums or social networks) were rarely used \cite{aalbers2011characteristics}, in this study the social features have been largely used by the participants. Further research is required to investigate whether this result is significant and related to the design of the tool.
%is that social networking forums are frequently used as a tool but rarely used by the participants, and thus are ineffective. Time may have come to incorporate modern features (i.e. web 2.0) into online lifestyle interventions. 

\subsection{Feasibility of online group-exercising}
Although not in scope, it is important to note that the design presented in this paper has been effective in enabling and engaging users to exercise from home, producing significant benefits in muscle strength and gait speed\footnote{Summary of adherence and physical outcomes at \url{http://gymcentral.net/trento.php}}.  
%Feeback from the Coach also reinforced the feasibility and potential benefits of the approach.


\subsection{Limitations}
\textbf{Different channels for Coach support}. The interactions of the Coach with the participants were scheduled to give the same type of support. However, in  absence of social features in the version of the app used by the Control group, the support was given by phone calls. This difference in the communication channel might have introduced a potential bias in the motivation to participate. 

\textbf{Sample size and gender imbalance}. Random variability, probably due to the small sample size, might have influenced the initial difference between groups in some of the measures. We also acknowledge the gender imbalance as a potential limitation to the generalisation of the results.





==> sections/results-behavior.tex <==
\subsection{Usage analysis and social interactions}
\begin{figure*}
\centering
  \includegraphics[width=1.8\columnwidth]{figures/behavoir-all}
  \caption{a)Time Spend by each user in Training, Social and persuasion, b)Contribution and productivity in the Bulletin board and Private messaging features, C)Trainee's application feature usage}~\label{fig:figureAll}
\end{figure*}
Participatns interaction with the trainee's application were recorded during the training program. The results inferred from the interaction logs reveals the actual usage of different features of the virtual gym.
We categorize these usage in three groups of i) \textit{training}, refering to the classroom that were desined to provide training exercises, ii) \textit{social}, referring to social interaction tools (e.g., locker-room, bulletin board, and proviate message) and iii) \textit{persuasion}, refering to the view and usage of the garden.
Figure \ref{fig:figureAll} \emph{a} depicts the time spent by participants in each of the three mentioned categories. Given that participants spent most of their times in the classroom exercising (Training=92\%, Social=6\%, Persuasion=1\%). However, the social features such as the locker room, bulletin board, and private messaging did not require a lot of time, yet the frequency of visiting is higher (Figure \ref{fig:figureAll} C) than the training features. Performance views however has smaller usage in both time spent and frequency of views.
Given the high usage of the social features, we analysed the contribution (How much the participant used the feature as a passive viewer) and productivity (how much the participants posted a message) of each participants. 
Figure \ref{fig:figureAll} B depicts the usage for both Bulletin board and the Private messaging feature. Notably, the productivity of the private messaging is higher but the deviation in the bulletin board post is lower and depicts a more common usage.


==> sections/results-feature.tex <==
\subsubsection{Feature Analysis}
Interaction logs obtained from the trainee's application demostrates the usage of all features by participants. From these, the usage of \textit{training features} (Agenda, Locker-room, classroom and performance view) along with the usage of \textit{social features} (bulletin Board, Private messaging, Invitation tool, and realtime interaction) were analysed.

\textit{Training Features.} Participants were given the option to enter to the virtual classroom for exercising from an agenda or through the virtual locker room. The agenda also shows the weekly training plan. Participants viewed the Agenda per user $(mean=21.09 views, S.D = 21.25)$ and per day $(mean=8.06 views, S.D = 6.29)$. The usage over time depicts a slight decline in using the agenda. However, most of the times, participants started the exercising through the virtual locker-room. Usage of the locker room per user $(mean=104.28 views, S.D = 39.40)$ and per day $(mean=40.20 views, S.D = 17.75)$ depicts that the locker-room were the entry room to most of the users equally despite that they could use the Agenda to enter to the classroom. In addition, participants use the performance monitoring per user $(mean=21.14 views, S.D = 19.80)$ and per day $(mean=8.26 views, S.D = 4.51)$. The deviation between the participants is relatively high, desmotrating that some participants were interested to follow their progress while some used it less. However the daily deviation is not significant and the usage by time did not have a significant raise or decline.  

\textit{Social Features.} Bulletin board were viewed per user $(mean=51.04 views, S.D = 40.14)$ and per day $(mean=19.00 views, S.D = 11.26)$. The usage over the 53 days of training depicts a raise in usage $(r^2 = 3.458E-3)$. Participants posted public posts to the bulletin board per user $(mean=3.61 posts, S.D = 5.21)$ and per day $(mean=1.41 posts, S.D = 1.68)$. Posting to the bulletin board over the 53 days of training had a decline $(r^2 = 0.042)$ over time. The results depicts consistence usage of the bulletin board feature. Despite the raise in viewing the bulletin board, participants tend to post less however.

Private messaging feature were viewed per user $(mean=35.33 views, S.D = 26.59)$ and per day $(mean=13.04 views, S.D = 8.21)$. The usage over the 53 days of training depicts a decline in usage $(r^2 = 0.042)$. Participants wrote private messages to the coach and other club members per user $(mean=10.33 message, S.D = 12.68)$ and per day $(mean=4.01 message, S.D = 2.91)$. Writing private message has also a decline $(r^2 = 0.011)$ over time. The deviation between participants usage depicts that some participants were highly more active than the others. In addition, the decline in the usage can refer to less need of using the private message to communicate with the coach and technician for help, since the feature were mainly used to communicate about the questions and challenges of the training. \textcolor{red}{How did you come to this conclusion? Qualitative analysis tells more about what was posted, but it's not longitudinal.}

Participants send invitations to their co-trainees per user $(mean=24.14 invitations, S.D = 74.26)$ and per day $(mean=9.37 invitations, S.D = 6.58)$. The high deviation between the number of intvitations sent by each participants depicts that while some of them were actively used the invitation tool to invite their co-trainees, some used it rarely or none. However, the usage over time did not change significantly. Beside this, only 1 participants tried the realtime interaction tool that was proviated in the locker room. The main reason is that participants spend a very little time in the locker room and the chances to meet other people were very low.

The overall analysis shows that the social group mainly used the training features. However, all participants were consistently using the social features and in particular the bulletin board. figure \ref{fig:figure4}


